Secure and Robust MIMO Transceiver for Multicast Mission Critical Communications

Mission-critical communications (MCC) involve all communications between people in charge of the safety of the civil society. MCC have unique requirements that include improved reliability, security and group communication support. In this paper, we propose a secure and robust Multiple-Input-Multiple-Output (MIMO) transceiver, designed for multiple Base Stations supporting multicast MCC in presence of multiple eavesdroppers. We formulate minimization problems with the Sum-Mean-Square-Error (SMSE) at legitimate users as an objective function, and a lower bound for the MSE at eavesdroppers as a constraint. Security is achieved thanks to physical layer security mechanisms, namely MIMO beamforming and Artificial Noise (AN). Reliability is achieved by designing a system which is robust to Channel State Information errors. They can be of known distribution or norm-bounded. In the former case, a coordinate descent algorithm is proposed to solve the problem. In the latter case, we propose an worst-case based iterative algorithm. Numerical results at physical layer and system level reveal the crucial role of robust designs for reliable MCC. We show the interest of both robust design and AN to improve the security gap. We show that full BS cooperation in preferred for highly secured and reliable MCC but dynamic clustering allows to trade-off security and reliability against capacity.

==> sections/case_studies.tex <==
% In this section we discuss various scenarios that and present the transceiver design. These are considered as special cases of the optimal robust design discussed in Sec~\ref{sec:proposed_design} which differs in availability of CSI of either transmitter and legitimate UEs or transmitters and eavesdroppers. For each case, either of stochastic or norm bounded errors can be considered for imperfections in CSI while formulating robust designs. Each of the possible case is discussed as follows:

%Case 1: Non-robust Transceiver design.% H non-robust G non-robust (Non-robust solution with known eves)

\textcolor{red}{What is the goal of this sub-section ? Isnt'it a special case of P1 ? If not what is the main difference ? }\textcolor{blue}{we can remove this section.}
In this section, we present the design of the transceivers and of the AN covariance matrix at the BSs and legitimate UEs while assuming the availability of perfect CSI for the channel between BSs and legitimate UEs. This will be referred as non-robust design. In this scenario, we have thus ${\bf \Delta}_{tl}=0$. Hence the MSE at the legitimate user $l$ can be given as:
\begin{eqnarray}
{\epsilon}_{l} &=& {\rm tr}({\bf I}) -%
{\rm tr}(\sum_{t=1}^{K_T}{\bf R}_{l}\widehat{\bf C}_{tl}{\bf V}_{t}) -%
{\rm tr}(\sum_{t=1}^{K_T}{\bf V}_{t}^{H}\widehat{\bf C}_{tl}^{H}{\bf R}_{l}^{H}) +%
{\rm tr}(\sum_{t=1}^{K_T}{\bf R}_{l}\widehat{\bf C}_{tl}{\bf V}_{t}{\bf V}_{t}^{H}\widehat{\bf C}_{tl}^{H}{\bf R}_{l}^{H}) \nonumber \\%
&+& {\rm tr}(\sum_{t=1}^{K_T}{\bf R}_{l}\widehat{\bf C}_{tl}{\bf W}_{t}\widehat{\bf C}_{tl}^{H}{\bf R}_{l}^{H}) +%
{\sigma}_{nl}^{2}{\rm tr}({\bf R}_{l}{\bf R}_{l}^{H}) \label{eq:epsl_non_robust}
\end{eqnarray}
It can be observed that \eqref{eq:epsl_non_robust} is a special case of~\eqref{eq:mse_leg_gen} in Appendix~\ref{app:robust} with $\chi_{l}=0$. Hence, we consider the similar optimization problem as defined in \eqref{P1} and obtain the desired transceiver matrices and AN filter. However, difference in the models considered while designing errors in eavesdroppers error (stochastic or NBE), it follows two different sub-cases, solution for which can be obtained as per the following proposition. \textcolor{red}{Sentence to be re-written.}

\begin{proposition}
Considering the perfect CSI at the legitimate users and imperfections in CSI at the eavesdroppers, the optimal precoder, AN covariance matrix, and receive filter verify the following equations:
\begin{eqnarray}
{\bf V}_{t} &=& ({\bf A}_{t})^{-1}\Big(\sum_{l=1}^{K_R}\widehat{\bf C}_{tl}^{H}{\bf R}_{l}^{H} - \sum_{e=1}^{K_E}\lambda_{e}\widehat{\bf G}_{te}^{H}{\bf E}_{e}^{H}\Big) \label{eq:pre_non_robust} \\
{\bf W}_t&=&{\bf B}_{t}/\sqrt{\mathbb[\rm tr({\bf B}_{t}{\bf B}_{t}^{H})]} \label{eq:an_non_robust} \\
{\bf R}_{l} &=& \Big(\sum_{t=1}^{K_T}{\bf V}_{t}^{H}\widehat{{\bf C}}_{tl}^{H}\Big)\Big(\sum_{t=1}^{K_T}\widehat{{\bf C}}_{tl}{\bf V}_{t}{\bf V}_{t}^{H}\widehat{{\bf C}}_{tl}^{H} +%
\sum_{t=1}^{K_T}\sigma_{zt}^{2}\widehat{{\bf C}}_{tl}{\bf W}_{t}{\bf W}_{t}^{H}\widehat{{\bf C}}_{tl}^{H} + {\sigma}_{nl}^{2}{\bf I} \label{eq:rec_non_robust}
\end{eqnarray}
where $\lambda_{e} \geq 0$, $\lambda_{t}^{'} and \geq 0$ are the Lagrangian multipliers, which are calculated such that the constraints $C1$ and $C2$ are satisfied respectively. $B_{t}$ and ${\bf A}_{t}$ are computed as:
\begin{eqnarray}
{\bf B}_{t}&=&{\bf I}-{\bf A}_{t}^{H}({\bf A}_{t}{\bf A}_{t}^{H})^{-1}{\bf A}_{t}),\nonumber
\end{eqnarray}
\begin{eqnarray}
{\bf A}_{t}&=& \sum_{l=1}^{K_R}\widehat{{\bf C}}_{tl}^{H}{\bf R}_{l}^{H}{\bf R}_{l}\widehat{\bf C}_{tl}-\sum_{e=1}^{K_E}{\lambda}_{e}\widehat{\bf G}_{te}^{H}{\bf E}_{e}^{H}{\bf E}_{e}\widehat{\bf G}_{te} -\sum_{e=1}^{K_E}{\lambda}_{e}{\sigma}_{te}^{2}{\rm tr}({\bf E}_{e}{\bf E}_{e}^{H})+ \lambda_{t}^{'}{\bf I}.\nonumber
\end{eqnarray}
\end{proposition}
\begin{IEEEproof}
With the perfect CSI knowledge at the
legitimate users and imperfect CSI information at the eavesdroppers, the complete proof for this specific design can be found in Appendix~\ref{app:alternativeW} with $\chi_{l}=0$ and $\chi_{e}=1$.
%When the channel knowledge for eavesdropper's is imperfect ${\bf \Delta}_{te}$ are modeled as stochastic errors with known error variance $\sigma_{te}$, the complete proof can be found in Appendix~\ref{app:robust} with $\chi_{l}=0$ and $\chi_{e}=1$. When the errors ${\bf \Delta}_{te}$ are modeled as norm-bounded errors, the complete proof can be found in Sec.~\ref{sec:norm_bound}
\textcolor{red}{not sure this is the correct corss-ref}\textcolor{blue}{~overall solution given in section \ref{sec:norm_bound}. I tried to make it clear now.} by first considering \eqref{PA} with $\chi_{l}=0$ and $\chi_{e}=1$ parameter settings followed by \eqref{PC}. The iterative algorithms~\ref{alg:iter_algo} and~\ref{alg:iter_norm} can be used with appropriate parameters to find the solution for respective channel error models. \textcolor{red}{Is it a proof?}
\end{IEEEproof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Case 1: H non-robust G robust (Non-robust solution with unknown eves)
% Proposition:

% Case 2: H non-robust G non-robust (Non-robust solution with known eves)
% Proposition:

% Case 3: H robust and G non-robust (Robust solution with known eves)
% Proposition:

==> sections/method.tex <==
\subsection{Non-Robust Design}
\subsection{Robust Design}
stochastic errors discussion for both robust and non robust

\subsection{Robust Transceiver Design}

An additional artificial noise (AN) vector ${\bf t}$ with zero mean and covariance matrix ${\bf T}={\mathbb E}[{{\bf t}}{{\bf t}}H]$ is sent by the BS to guarantee security. Thus the signal transmitted from ${i}^{th}$ BS can be given as:
\begin{eqnarray}
{\bf x}_{i} = {\bf V}_{i}{\bf d} + {\bf w}_{i}
\end{eqnarray}

${\bf w}_{i}$ vector is zero mean and covariance matrix $\mathbb{E}[{\bf w}{\bf w}^{H}]$ is artificial noise sent by the BS to guarantee security. Consequently, the received signal at intended user $j$ is given by
\begin{eqnarray}
{\bf y}_{j} = \sum_{i=1}^{j_1}{\bf C}_{ij}{\bf V}_{i}{\bf d} + \sum_{i=1}^{K_1}{\bf C}_{ij}{\bf w}_{i} + {\bf n}_{j}
\end{eqnarray}

Thus, the estimate of the transmitted data at user $j$ can now be given by:

\begin{eqnarray}
\widehat{\bf d}_{j} = \sum_{i=1}^{j_1}{\bf R}_{j}{\bf C}_{ij}{\bf V}_{i}{\bf d} + \sum_{i=1}^{j_1}{\bf R}_{j}{\bf C}_{ij}{\bf w}_{i} + {\bf R}_{j}{\bf n}_{j}.
\end{eqnarray}

During each transmission from the BS, the eavesdropper E can overhear signal. Let the ${\bf G}_{iE}$ be the channel between the $i$-th BS and Eve. As it is impractical to have the perfect CSI knowledge about the Eve's channel as eavesdroppers CSI is expected to be much less accurate as compared to legitimate UEs CSI. We assume to have only imperfect knowledge about eavesdroppers CSI. We consider the norm-bounded error (NBE) model to characterize Eve's channel. Hence, following this the received signal at the eavesdropper can be given as:
\begin{eqnarray}
{\bf y}_{e} = {\bf G}_{ie}{\bf V}_{i}{\bf d} + {\bf G}_{ie}{\bf w}{i} + {\bf n}_{e}
\end{eqnarray}

where ${\bf G}_{ie} = \widehat{\bf G}_{ie} + {\bf \Delta}_{ie}$. ${\bf \Delta}_{ie}$ is considered to be norm bounded without any statistical knowledge about errors in CSI such that

\begin{eqnarray}
\mathcal{G}_{ie} = \{{\bf \Delta}_{ie} : {||{\bf \Delta}_{ie}||}^{2} \leq {\bf \delta}_{ie}\}
\end{eqnarray}

where, ${bf \delta}_{ie}$ denotes the radius of uncertainty region.  

The mean square error at the $j$-th legitimate user can be given as follows:
\begin{IEEEeqnarray}{lll}
{\epsilon}_{j} &=& \mathbb{E}||\bf{d}-\bf{d}_{j}^{H}||^{2} \nonumber
\\
&=&\mathbb {E}(||d-(\sum_{i=1}^{K_1}{\bf R}_{j}{\bf C}_{ij}{\bf V}_{i}{\bf d} + \sum_{i=1}^{K_1}{\bf R}_{j}{\bf C}_{ij}{\bf w}_{i} + {\bf R}_{j}{\bf n}_{j})||^{2})\nonumber \\
&=&\mathbb {E}({\rm tr}(d-(\sum_{i=1}^{K_1}{\bf R}_{j}{\bf C}_{ij}{\bf V}_{i}{\bf d} + \sum_{i=1}^{K_1}{\bf R}_{j}{\bf C}_{ij}{\bf w}_{i} + {\bf R}_{j}{\bf n}_{j}))(d-(\sum_{i=1}^{K_1}{\bf R}_{j}{\bf C}_{ij}{\bf V}_{i}{\bf d} + \sum_{i=1}^{K_1}{\bf R}_{j}{\bf C}_{ij}{\bf w}_{i} \nonumber \\
&&+ {\bf R}_{j}{\bf n}_{j}))^{H})\nonumber \\
{\epsilon}_{j} &=& {\rm tr}\bigg(I-\sum_{i=1}^{K_1}{\bf V}_{i}^{H}{\bf C}_{ij}^{H}{\bf R}_{j}^{H} - \sum_{i=1}^{K_1}{\bf R}_{j}{\bf C}_{ij}{\bf V}_{i}  + \sum_{i=1}^{K_1}{\bf R}_{j}{\bf C}_{ij}{\bf V}_{i}{\bf V}_{i}^{H}{\bf C}_{ij}^{H}{\bf R}_{j}^{H} \nonumber \\
&& + \sum_{i=1}^{K_1}{\bf R}_{j}{\bf C}_{ij}{\bf W}_{i}{\bf C}_{ij}^{H}{\bf R}_{j}^{H} + \sigma_{nj}^{2}{\bf R}_{j}{\bf R}_{j}^{H}\bigg) 
\end{IEEEeqnarray}

The MSE at eavesdropper can be given as:
\begin{IEEEeqnarray}{lll}
{\epsilon}_{e} &=& \mathbb{E}||{\bf d}-{\bf d}_{e}^{H}||^{2} \nonumber
\\
&=&\mathbb {E}(||d-(\sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf V}_{i}{\bf d} + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf w}_{i} + {\bf E}_{e}{\bf n}_{e})||^{2})\nonumber \\
&=&\mathbb {E}({\rm tr}(d-(\sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf V}_{i}{\bf d} + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf w}_{i} + {\bf E}_{e}{\bf n}_{e}))\nonumber \\
&&(d-(\sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf V}_{i}{\bf d} + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf w}_{i} + {\bf E}_{e}{\bf n}_{e}))^{H})\nonumber \\
% &=&\mathbb {E}(tr(d-(\sum_{i=1}^{K_1}{\bf E}_{e}({\bf G}_{ie}+{\bf \Delta}_{ie}){\bf V}_{i}{\bf d} + \sum_{i=1}^{K_1}{\bf E}_{e}({\bf G}_{ie}+{\bf \Delta}_{ie}){\bf w}_{i} + {\bf E}_{e}{\bf n}_{e}))\nonumber \\
% &&(d-(\sum_{i=1}^{K_1}{\bf E}_{e}({\bf G}_{ie}+{\bf \Delta{ie}}){\bf V}_{i}{\bf d} + \sum_{i=1}^{K_1}{\bf E}_{e}({\bf G}_{ie}+{\bf \Delta}_{ie}){\bf w}_{i} + {\bf E}_{e}{\bf n}_{e}))^{H})\nonumber \\
{\epsilon}_{e} &=& {\rm tr}\bigg(I-\sum_{i=1}^{K_1}{\bf V}_{i}^{H}{\bf G}_{ie}^{H}{\bf E}_{e}^{H} - \sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf V}_{i}  + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf V}_{i}{\bf V}_{i}^{H}{\bf G}_{ie}^{H}{\bf E}_{e}^{H} \nonumber \\
&& + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf W}_{i}{\bf G}_{ie}^{H}{\bf E}_{e}^{H} + \sigma_{ne}^{2}{\bf E}_{e}{\bf E}_{e}^{H}\bigg) 
\end{IEEEeqnarray}

Thus the optimization problem can be mathematically formulated as,

\begin{IEEEeqnarray}{lll}
\min_{\{\mathbf{V}_i\},\{\mathbf{W}_i\},\{\mathbf{R}_j\}} & \sum_{j=1}^{K_2}{\rm \epsilon}_{j} \label{eq:minprob},\\
\text{s.t.} & {\rm \epsilon}_{e} \geq \Gamma \nonumber\\ &
{P_{i}}\leq P_T, \; i=1,...,K_1,\nonumber\\
& {\bf \Delta}_{ie} \in \mathcal{R}_{{\bf \Delta}_{ie}}
\label{eq:constraint}
%{\rm tr}(\mathbf{V}_i\mathbf{V}_i^H)\leq P_T, \; i=1,...,K_1, \label{eq:constraint}
\end{IEEEeqnarray}

where, 
\begin{IEEEeqnarray}{lll}
{P}_{i}&=&\mathbb{E}[||{\bf x}_{i}{\bf x}_{i}^{H}||]\nonumber \\
& =& \mathbb{E}[{\rm}{Tr}({\bf x}_{i}{\bf x}_{i}^{H})]\nonumber \\
& =& \mathbb{E}[{\rm}{Tr}(({\bf V}_{i}{\bf d} + {\bf w}_{i})({\bf V}_{i}{\bf d} + {\bf w}_{i})^{H})]\nonumber \\
&=&{\rm}{Tr}({\bf V}_{i}{\bf V}_{i}^{H}+{\bf W}_{i})
\end{IEEEeqnarray}
Thus the optimization problem is equivalent to:

\begin{IEEEeqnarray}{lll}
\label{eq:minprob}
\min_{\{\mathbf{V}_i\},\{\mathbf{W}_i\},\{\mathbf{R}_j\}} && \sum_{j=1}^{K_2}{\rm \epsilon}_{j} ,\\
\text{s.t.} && \min_{\{\mathbf{\Delta}_{ie} \in{\mathcal{R}_{\bf \Delta}\}}} {\rm \epsilon}_{e} \geq \Gamma  \nonumber\\
&&{\rm}{Tr}({\bf V}_{i}{\bf V}_{i}^{H}+{\bf W}_{i})\leq P_T, \; i=1,...,K_1,\nonumber 
\end{IEEEeqnarray}

Problem A: Computation of precoder ${\bf V}_{i}$, receive filters precoder ${\bf R}_{j}$ and filter precoder ${\bf W}_{i}$ for given channel errors ${\bf \Delta}_{ie}$.

Mathematically the problem can be formulated as:
\begin{IEEEeqnarray}{lll}
\label{eq:minprob}
\min_{\{\mathbf{V}_i\},\{\mathbf{W}_i\},\{\mathbf{R}_j\}} && \sum_{j=1}^{K_2}{\rm \epsilon}_{j} , \\
\text{s.t.} &&  {\rm \epsilon}_{e} \geq \Gamma  \nonumber\\
&&{\rm}{Tr}({\bf V}_{i}{\bf V}_{i}^{H}+{\bf w}_{i})\leq P_T, \; i=1,...,K_1,\nonumber
\end{IEEEeqnarray}

Problem B: Computation of worst case channels, i.e., Computation of worst case channels/ channel vectors that belong to the uncertainty region and minimize total legitimate users mean square error.

\begin{IEEEeqnarray}{lll}
&&\min_{{\bf \Delta}_{ie} \forall 1 \leq i \leq K1} \epsilon_{e} \\
&&\text{s.t.} \nonumber \\
&& ||{\bf \Delta}_{ie}||^{2} \leq \sigma_{ie} \quad \forall 1 \leq i \leq K1 \nonumber
\end{IEEEeqnarray}
Where MSE at eve-dropper with channel errors can be written as:
\begin{IEEEeqnarray}{lll}
&&\epsilon_{e} = tr\bigg(I-\sum_{i=1}^{K_1}{\bf V}_{i}^{H}{\bf G}_{ie}^{H}{\bf E}_{e}^{H} - \sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf V}_{i}  + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf V}_{i}{\bf V}_{i}^{H}{\bf G}_{ie}^{H}{\bf E}_{e}^{H} \nonumber \\
&& + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf G}_{ie}{\bf W}_{i}{\bf G}_{ie}^{H}{\bf E}_{e}^{H} + \sigma_{ne}^{2}{\bf E}_{e}{\bf E}_{e}^{H}\bigg) \nonumber \\
&&= tr\bigg(I-\sum_{i=1}^{K_1}{\bf V}_{i}^{H}(\widehat{{\bf G}}_{ie}+{\bf \Delta}_{ie})^{H}{\bf E}_{e}^{H} - \sum_{i=1}^{K_1}{\bf E}_{e}(\widehat{{\bf G}}_{ie}+{\bf \Delta}_{ie}){\bf V}_{i} \nonumber \\
&& + \sum_{i=1}^{K_1}{\bf E}_{e}(\widehat{{\bf G}}_{ie}+{\bf \Delta}_{ie}){\bf V}_{i}{\bf V}_{i}^{H}(\widehat{{\bf G}}_{ie}+{\bf \Delta}_{ie})^{H}{\bf E}_{e}^{H} + \sum_{i=1}^{K_1}{\bf E}_{e}(\widehat{{\bf G}}_{ie}+{\bf \Delta}_{ie}){\bf W}_{i}(\widehat{{\bf G}}_{ie}+{\bf \Delta}_{ie})^{H}{\bf E}_{e}^{H} + \sigma_{ne}^{2}{\bf E}_{e}{\bf E}_{e}^{H}\bigg) \nonumber \\
&&= tr\bigg(I-\sum_{i=1}^{K_1}{\bf V}_{i}^{H}\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H} - \sum_{i=1}^{K_1}{\bf E}_{e}\widehat{{\bf G}}_{ie}{\bf V}_{i} -\sum_{i=1}^{K_1}{\bf V}_{i}^{H}{\bf \Delta}_{ie}^{H}{\bf E}_{e}^{H} - \sum_{i=1}^{K_1}{\bf E}_{e}{\bf \Delta}_{ie}{\bf V}_{i} + \sum_{i=1}^{K_1}{\bf E}_{e}\widehat{{\bf G}}_{ie}{\bf V}_{i}{\bf V}_{i}^{H}\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H} \nonumber \\
&&  + \sum_{i=1}^{K_1}{\bf E}_{e}\widehat{{\bf G}}_{ie}{\bf V}_{i}{\bf V}_{i}^{H}{\bf \Delta}_{ie}^{H}{\bf E}_{e}^{H} + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf \Delta}_{ie}{\bf V}_{i}{\bf V}_{i}^{H}\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H} + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf \Delta}_{ie}{\bf V}_{i}{\bf V}_{i}^{H}{\bf \Delta}_{ie}^{H}{\bf E}_{e}^{H} + \sum_{i=1}^{K_1}{\bf E}_{e}\widehat{{\bf G}}_{ie}{\bf W}_{i}\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}   \nonumber \\
&&  + \sum_{i=1}^{K_1}{\bf E}_{e}\widehat{{\bf G}}_{ie}{\bf W}_{i}{\bf \Delta}_{ie}^{H}{\bf E}_{e}^{H} + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf \Delta}_{ie}{\bf W}_{i}\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H} + \sum_{i=1}^{K_1}{\bf E}_{e}{\bf \Delta}_{ie}{\bf W}_{i}{\bf \Delta}_{ie}^{H}{\bf E}_{e}^{H} + \sigma_{ne}^{2}{\bf E}_{e}{\bf E}_{e}^{H}\bigg)
\end{IEEEeqnarray}

For simplicity, we discard the second and higher order terms of ${\bf \Delta}_{ie}$. Also, let $\overline{\epsilon}_{e}$ represents the MSE at eves-dropper considering ${\bf \Delta}_{ie}$ to be zero. Hence, estimation of MSE caused by a specific BS can be written as:

\begin{IEEEeqnarray}{lll}
\epsilon_{ie} &\approx& \overline{\epsilon}_{ie} - tr({\bf V}_{i}^{H}{\bf \Delta}_{ie}^{H}{\bf E}_{e}^{H}) - tr({\bf E}_{e}{\bf \Delta}_{ie}{\bf V}_{i}) + tr({\bf E}_{e}\widehat{{\bf G}}_{ie}{\bf V}_{i}{\bf V}_{i}^{H}{\bf \Delta}_{ie}^{H}{\bf E}_{e}^{H}) + tr({\bf E}_{e}{\bf \Delta}_{ie}{\bf V}_{i}{\bf V}_{i}^{H}\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}) \nonumber \\
&&+ tr({\bf E}_{e}\widehat{{\bf G}}_{ie}{\bf W}_{i}{\bf \Delta}_{ie}^{H}{\bf E}_{e}^{H}) + tr({\bf E}_{e}{\bf \Delta}_{ie}{\bf W}_{i}\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H})
\end{IEEEeqnarray}
Reformulating only the part of MSE with ${\bf \Delta}_{ie}$.
\begin{IEEEeqnarray}{lll}
\label{eq:mse_eve_appx}
\epsilon_{ie} &\approx& \overline{\epsilon}_{ie} - tr(({\bf V}_{i}{\bf E}_{e}{\bf \Delta}_{ie}) + ({\bf V}_{i}{\bf E}_{e}{\bf \Delta}_{ie})^{H}) + tr({\bf E}_{e}\widehat{{\bf G}}_{ie}({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i}){\bf \Delta}_{ie}^{H}{\bf E}_{e}^{H})  \nonumber \\
&&+ tr({\bf E}_{e}{\bf \Delta}_{ie}({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i})\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}) \nonumber \\
&\approx& \overline{\epsilon}_{ie} - tr(({\bf V}_{i}{\bf E}_{e}{\bf \Delta}_{ie}) + ({\bf V}_{i}{\bf E}_{e}{\bf \Delta}_{ie})^{H}) + tr((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})^{H}({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i}))  \nonumber \\
&&+ tr((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i})) \nonumber \\
&\approx& \overline{\epsilon}_{ie} - tr(({\bf V}_{i}{\bf E}_{e}{\bf \Delta}_{ie}) + ({\bf V}_{i}{\bf E}_{e}{\bf \Delta}_{ie})^{H}) + tr(((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})^{H} + (\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie}))({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i}))  \nonumber \\
\end{IEEEeqnarray}
Using the inner product and Cauchy-inequality properties of trace
\begin{IEEEeqnarray}{lll}
[tr(((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})^{H} &+& (\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie}))({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i}))]^{2} \leq \nonumber \\
&&[tr(((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})^{H} + (\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})))]^{2} [tr({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i})]^{2} \nonumber
\end{IEEEeqnarray}
taking square root on both the sides
\begin{IEEEeqnarray}{lll}
tr(((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})^{H} &+& (\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie}))({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i})) \leq \nonumber \\
&&tr(((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})^{H} + (\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie}))) tr({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i}) \nonumber
\end{IEEEeqnarray}
Considering the worst-case solution
\begin{IEEEeqnarray}{lll}
tr(((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})^{H} &+& (\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie}))({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i})) = \nonumber \\
&&tr(((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})^{H} + (\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie}))) tr({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i}) \nonumber
\end{IEEEeqnarray}
Hence replacing in eqn \ref{eq:mse_eve_appx}, we get
\begin{IEEEeqnarray}{lll}
&\approx& \overline{\epsilon}_{ie} - tr(({\bf V}_{i}{\bf E}_{e}{\bf \Delta}_{ie}) + ({\bf V}_{i}{\bf E}_{e}{\bf \Delta}_{ie})^{H}) + tr(((\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})^{H} + (\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie}))) tr({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i}) \nonumber
\end{IEEEeqnarray}
Considering only the Real value from the equation, we can say that
\begin{IEEEeqnarray}{lll}
\mathbb{R}({\bf A})^{H} &=& \mathbb{R}({\bf A})^{T} \nonumber \\
\mathbb{R}tr({\bf A}) &=& \mathbb{R}tr({\bf A}^{T}) = \mathbb{R}tr({\bf A}^{H}) \nonumber
\end{IEEEeqnarray}
Hence, the MSE estimate can be written as:
\begin{IEEEeqnarray}{lll}
&\approx& \overline{\epsilon}_{ie} - 2\mathbb{R}tr({\bf V}_{i}{\bf E}_{e}{\bf \Delta}_{ie}) + 2\mathbb{R}tr(\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H}{\bf E}_{e}{\bf \Delta}_{ie})tr({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i}) \nonumber \\
&\approx& \overline{\epsilon}_{ie} + 2\mathbb{R}tr((B\widehat{{\bf G}}_{ie}^{H}{\bf E}_{e}^{H} - {\bf V}_{i}){\bf E}_{e}{\bf \Delta}_{ie})
\end{IEEEeqnarray}
where $B = tr({\bf V}_{i}{\bf V}_{i}^{H} + {\bf W}_{i})$, Using Cauchy-inequalities and solving it for worst case scenario
\begin{IEEEeqnarray}{lll}
{\bf \Delta}_{ie} = \frac{\sigma_{ie}}{||{\bf E}_{e}^{H}(B{\bf E}_{e}\widehat{{\bf G}}_{ie} -  {\bf V}_{i}^{H})||} (B{\bf E}_{e}\widehat{{\bf G}}_{ie} -  {\bf V}_{i}^{H})
\end{IEEEeqnarray}


\subsection{Problem Formulation}
